Deep Non-rigid Structure-from-Motion Revisited: Canonicalization and Sequence Modeling

Non-Rigid Structure-from-Motion (NRSfM) is a classic 3D vision problem, where a 2D sequence is taken as input to estimate the corresponding 3D sequence. Recently, the deep neural networks have greatly advanced the task of NRSfM. However, existing deep NRSfM methods still have limitations in handling the inherent sequence property and motion ambiguity associated with the NRSfM problem. In this paper, we revisit deep NRSfM from two perspectives to address the limitations of current deep NRSfM methods : (1) canonicalization and (2) sequence modeling. We propose an easy-to-implement per-sequence canonicalization method as opposed to the previous per-dataset canonicalization approaches. With this in mind, we propose a sequence modeling method that combines temporal information and subspace constraint. As a result, we have achieved a more optimal NRSfM reconstruction pipeline compared to previous efforts. The effectiveness of our method is verified by testing the sequence-to-sequence deep NRSfM pipeline with corresponding regularization modules on several commonly used datasets.

==> text/0_Abstract.tex <==
\begin{abstract}

% Prior non-rigid 3D reconstruction efforts have typically relied on the strong inference capabilities of networks that regressing corresponding 3D shapes from individual frame of 2D observations. Nevertheless, such estimation pipelines rarely consider the relationship among the members of the reconstructed sequence of deformation shapes, when in fact, the non-rigid deformation process itself can provide strong constraints on the reconstructed network. This paper discusses the structural properties of sequence data in the NRSfM task and the role this property plays in the computational process. Based on this, we propose a series of methods that can effectively impose the sequence structure property as a constraint in the deep NRSfM pipeline, so that the structural characteristics of the sequence data itself can help the network to better estimate the non-rigid shape, thus to achieve a sequence-to-sequence deep non-rigid reconstruction scheme. Finally, comparative experiments on different datasets with several frame-by-frame approaches validate the correctness of the assumptions.


% In previous work on non-rigid 3D reconstruction, most have chosen to constrain the solution process using both alignment-based regular and low-rank-based regular ideas, but little work has pointed out the correlation between the two. Moreover, many reconstruction algorithms based on deep learning methods directly adopt the above mentioned regularization as loss functions, with little consideration of the relationship between these regularization and the data structure. Therefore, in this paper, we will first discuss the relationship between alignment regularity and low-rank regularity, explore the existence of complementary relationship between them in the constrained solution space, and the method of introducing the above two regular constraints directly in the inference process based on the characteristics of sequence data and the complementary nature of the two in the case of sequence input, where the regular constraints in the inference can form a stronger constraint effect than the loss function. Finally, the sequence-to-sequence reconstruction pipeline obtained based on the above principles is tested on several data sets to verify the correctness of the statements about the above.

Non-Rigid Structure-from-Motion (\textbf{NRSfM}) is a classic 3D vision problem, where a 2D sequence is taken as input to estimate the corresponding 3D sequence. Recently, the deep neural networks have greatly advanced the task of NRSfM. However, existing deep NRSfM methods still have limitations in handling the inherent sequence property and motion ambiguity associated with the NRSfM problem. In this paper, we revisit deep NRSfM from two perspectives to address the limitations of current deep NRSfM methods : \textbf{(1)} canonicalization and \textbf{(2)} sequence modeling.
% Firstly, we propose to conduct \emph{per-sequence canonicalization} rather than per-dataset canonicalization.
% Firstly, we propose a per-sequence rather than per-dataset canonicalization based on an easy-to-implement GPA Layer. 
% Secondly, we revisit two regularization schemes in modeling sequence structure and mitigating the ambiguity, to explore the complementary roles in delineating the correct solution space.
We propose an easy-to-implement per-sequence canonicalization method as opposed to the previous per-dataset canonicalization approaches. With this in mind, we propose a sequence modeling method that combines temporal information and subspace constraint. As a result, we have achieved a more optimal NRSfM reconstruction pipeline compared to previous efforts. The effectiveness of our method is verified by testing the sequence-to-sequence deep NRSfM pipeline with corresponding regularization modules on several commonly used datasets.

%       , and, based on this, to design a module that can effectively exploit the role of the two regularization schemes.

%     While the sequence property has been widely exploited in the traditional optimization framework, its deep counterpart has been seldom investigated. It is worth-noting that until very recently the sequence modeling has been introduced. This is mainly due to the difficulties in XXX. 

%   Per-frame Canonicalization

%   Sequence Canonicalization

%   inherent shape-motion ambiguity

%   Our method consists of \textbf{1)} \textbf{2)} \textbf{3)}

%      While incremental reconstruction systems have tremendously advanced in all regards, robustness, accuracy, completeness, and scalability remain the key problems towards building a truly general-purpose NRSfM pipeline



%          Traditional Non-Rigid Structure-from-Motion (\textbf{NRSfM}) methods typically model the sequence as a whole, so that the highly underdetermined problem can be solved by factorization framework. 


%           Within the deep NRSfM methods, sequence structure modeling can introduce the sequence structure feature into the training process or inference process, so that the network can effectively use the reconstructed target context information and thus improve the accuracy of the final reconstruction results.
%          Currently, there are two more commonly used ideas in mainstream work for constructing constraints on sequence modeling: the canonicalization regular scheme, which reduces the ambiguity of non-decoupled motions, and the low-rank regular scheme, which constrains the shape sequence matrix to be of low rank. 
%    These two modeling schemes have been studied from different aspects on the data characteristics of non-rigid shape sequences, but little work has been done to analyze the similarities and differences in the underlying logic of the two schemes.

% Currently, mainstream work typically constructs constraints on shape sequences using either a canonicalization regular scheme that reduces motion ambiguity or a low-rank regular scheme that constrains the numerical characteristics of shape sequences. 

% When constructing NRSfM sequence models, either alignment-based or low-rank-based regularity schemes are usually used to introduce the modeling of non-rigid reconstruction problem features, and the algorithms usually have different computational processes depending on the used regularity schemes. However, little work has been done to discuss the similarities and differences in the underlying logic of the two regularization schemes and the resulting complementary in functionality. 
%and the functional complementarities that result from them. 

\end{abstract}


==> text/1_Introduction.tex <==
\section{Introduction}
\label{Introduction}

% Non-rigid Structure from Motion is one of the classic problem in 3D computer vision society, plenty of work has been done in this field. The rigid reconstruction tasks have static reconstruction objectives, both classical mathematical methods~\cite{bregler2000recovering,dai2014simple,zhu2014complex} and recent network-based 
% methods~\cite{novotny2019c3dpo,kong2020deep,park2020procrustean,zeng2022mhr} that can build solution models based on combinations of various multi-view geometric constraints~\cite{}. 
% In contrast, most of the multi-view geometric constraints no longer prevail in NRSfM due to the deformation properties of the non-rigid object. For this reason, although the rigid reconstruction problem and the non-rigid reconstruction problem can both be described uniformly as a matrix decomposition problem\cite{bregler2000recovering,dai2014simple} that decomposes the shape matrix and the rigid transformation matrix from the observation matrix, yet the difficulty of their solutions differs significantly due to the available constraints.  

% The reconstruction task can be modeled as a matrix decomposition problem\cite{tomasi1992shape} which can be solved by solving a set of linear equations. Unfortunately, the non-rigid reconstruction task does not take a large number of available constraints based on multi-view geometry like the rigid reconstruction. This results in very few linearly independent constraints in the non-rigid reconstruction task, not sufficient to cover all the variables to be solved. This leads to a highly underdetermined solution process.Earlier work to cope with this problem usually starts with a parameterized template\cite{blanz1999morphable} of the object, this makes the problem solvable by artificially setting a strong prior. 

Non-Rigid Structure-from-Motion (NRSfM) is one of the classical tasks in 3D computer vision, which aims at recovering the 3D deforming shape sequences from 2D observation sequences.
% The main difference between this task and the ordinary SfM is that the reconstructed object is not static, so the classical multi-view geometry model is not applicable to this scenario.
There has been a lot of work trying to construct a reasonable model for this task. Various traditional mathematical methods~\cite{akhter2008nonrigid, akhter2009defense, dai2014simple,zhu2014complex} based on the factorization framework\cite{tomasi1992shape}, represented by Bregler~\etal~\cite{bregler2000recovering}, have produced remarkable results in modeling the deformation sequences.

Along with the rise of machine learning techniques and the advantages shown by neural network models in terms of inference speed and computational accuracy, more people have started to combine deep learning with non-rigid 3D reconstruction~\cite{novotny2019c3dpo, kong2020deep, wang2020deep, zeng2022mhr, wang2021paul, zeng2021pr, park2020procrustean}, and some progress has been made. These methods have certain advantages over traditional methods in terms of computational accuracy, inference speed, and handling of shape ambiguity. However, they also encountered the same problem as traditional methods, namely motion ambiguity, where ambiguity interferes with the direction of convergence of the network, which in turn leads to poor estimation results. And to cope with this problem, C3dpo\cite{novotny2019c3dpo} proposes the concept of transversal property and designs the canonicalization network for suppressing the ambiguity over the whole dataset. On the other hand, PRN\cite{park2020procrustean} represents a sequential regularization method based on Procrustean Analysis(PA) and an elegant training method that eliminates the need for the network to perform complex PA during inference. However, the implementation and computational complexity of this network in training are relatively high. At the same time, the backbone network of these methods\cite{novotny2019c3dpo,park2020procrustean,sidhu2020neural,zeng2021pr} only performs lifting on 2D observations and lacks modeling of continuous 2D observations sequences.

% However, most of these methods use single-frame lifting to regress the corresponding 3D deforming shapes, and other methods that use sequence input do not model specifically for targeting sequences. The modeling of deformation shape sequences, which is most valued in traditional mathematical modeling, is neglected and the ability to use sequence structure information is lost.

Recently, Deng~\etal\cite{deng2022deep}({denoted as Seq2Seq}) designs sequence reconstructing module 
% that can be applied to deep learning pipelines 
by referring to the traditional mathematical modeling of sequences, and has achieved promising results. However, instead of tackling canonicalization in a sequential manner, this method follows \cite{novotny2019c3dpo} and deals with the problem over the entire dataset. In addition, this method models the sequence with little consideration of the positional information in the sequence structure, and only an absolute positional encoding bias is used to inject temporal information into the sequence reconstruction process.

In this paper, we propose to revisit the deep NRSfM problem. We argue that dealing with shape ambiguity in a \emph{sequence-by-sequence} manner is more effective than over the entire dataset, reducing ambiguity's effect on the estimation results. We propose a sequential canonicalization based on General Procrustean Analysis(GPA). This method centers on a parameter-free GPA layer, which avoids high training overhead and eliminates the need for complex GPA operations during inference.
% We therefore, refer to the Generalized Procrustean Analysis(GPA) and design a easy-to-implementation GPA layer for sequential canonicalization. 
% , and there is no need to additionally add any new loss function.
% Also, We argue that the temporal bias term can be of limited use when not used in conjunction with temporal-related downstream constraints, but additional downstream constraints will increase the difficulty of network training.
% We argue that using temporal bias alone to introduce temporal information for sequence reconstruction is insufficient, because there is no guarantee that the network will understand what the bias represents. Therefore, we propose a sequence reconstruction weight calculation that can effectively incorporate the temporal information.
And in conjunction with the canonicalization for sequences, we design a sequence modeling method that can utilize sequence temporal more effectively. We argue that using temporal bias alone to introduce temporal information for sequence reconstruction is insufficient, because there is no guarantee that the network will understand what the bias represents.

Our main contributions are summarized as follows:
\begin{itemize}
% \item A parameter-free GPA layer that is capable of sequence-by-sequence canonicalization, effectively reducing the impact of the inherent ambiguity of NRSfM on estimation accuracy;
\item A sequence-by-sequence canonicalization method with an easy-to-implement GPA Layer, effectively reducing the impact of the inherent ambiguity of NRSfM on estimation accuracy;
\item A method that can efficiently incorporate temporal information to reconstruct non-rigid sequences for better shape sequence estimation results; 
\item We conducted experiments on a substantial amount of data, and the results confirm the validity of our method in most scenarios.
\end{itemize}

% \YC{the above paragraph has not been finished with details and highlights, some conclusion or contributions summarized are needed in the introduction section.}

% A strong priori, on the other hand, means that the application scenario is restricted, which makes such methods available only on specific categories. For arbitrary objects, Bregler \etal~\cite{bregler2000recovering} propose factorization framework that models deforming object as a linear combination of a set of basis. Factorization framework laid the foundation for mathematical methods to solve the NRSfM problem, and plenty of subsequent methods have been derived from this framework. However, Xiao \etal~\cite{xiao2004closed} proves that factorization is still underdetermined and the ambiguity of the solution process leads to a loss of accuracy, nevertheless, this work also simultaneously proposes a less strong prior from the perspective of numerical solution, allowing the solution accuracy to be improved while the method can be applied to more scenarios.

% The deep-based method~\cite{novotny2019c3dpo, kong2020deep, zeng2022mhr}, focuses on representing the optimization objective in a data-driven manner and designing the neural network to learn the a priori properties in the data in an implicit form. The deep-based method has advantages over traditional optimization methods in terms of inference speed and solution accuracy, but lacks in the exploration of the principles of the reconstruction problem itself. As mentioned in the previous section, the various explicit priors in the data structure, and the underlying logic of these designed priors, are rarely explored in deep-based methods, which by default assume these concepts being implicitly embedded in the weight of neural network during data-driven learning.

% We argue that two key points that often arise in nrsfm problems, ambiguity handling, and low-rankness are actually correlated, and this correlation is reflected when dealing with non-rigid deformation shapes in a sequential manner. That is, when non-rigid reconstruction problems are explored in terms of sequences, the ambiguity treatment can effectively guarantee the low-rankness of the sequences, and in turn low-rankness can effectively reduce the problem of accuracy loss due to ambiguity.On this basis, we propose a computational module that can effectively reduce the ambiguity and an accompanying canonical module that constrains the low-rankness, and combine the advantages of deep learning techniques in mapping fitting to obtain a pipeline that can solve sparse non-rigid 3D reconstruction in the form of sequence-to-sequence.


==> text/2_Relatedwork.tex <==
\section{Related Work}
% \subsection{Non-Rigid Structure from Motion}
% Non-Rigid-Structure-from-Motion(NRSfM) is a classic problem in computer vision, which aims to recover the sequence of 3D structure and camera motion from a series of 2D annotations. This problem is highly ill-posed, and in the following we briefly review the traditional and deep learning methods for NRSfM.

\subsection{Classical NRSfM Methods}
Bregler~\etal~\cite{bregler2000recovering} first introduced factorization framework~\cite{tomasi1992shape} for Non-rigid Structure-from-Motion.
% the matrix decomposition method in rigid-structure-from-motion into the field of non-rigid 3D reconstruction, which modeling the 3D structure as a linear combination of a series of shape bases, and decomposing the observation matrix according to the camera projection model to restore the camera motion and 3D shapes. 
Xiao~\etal~\cite{xiao2004closed} pointed out that the recovery of shape basis has inherent ambiguity problems. Akhter~\etal~\cite{akhter2009defense} showed that the non-rigid 3D shapes can be recovered uniquely by suitable optimization method under the orthogonal constraint. Subsequent researchers have proposed many effective NRSfM methods, including using DCT basis to recover motion trajectory\cite{akhter2008nonrigid, gotardo2011computing}, using low-rank constraint to regularize 3D structure recovery\cite{paladini2010sequential, dai2014simple, kumar2020non, kumar2022organic}, using hierarchical prior\cite{torresani2008nonrigid}, using union-of-subspace constraint\cite{zhu2014complex, kumar2016multi, kumar2017spatio}, using procrustean alignment to refine camera motion\cite{lee2013procrustean, Lee_2014_CVPR, park2017procrustean}, using consensus prior\cite{cha2019reconstruct}, using manifold to model non-rigid 3D surface\cite{kumar2018scalable, parashar2017, parashar2020local}, and many other quintessential methods\cite{marques2008optimal, paladini2009factorization, garg2013dense, simon2016kronecker, agudo2016recovering}.

% Researchers have proposed solutions for NRSfM from different perspectives, among which there are some mainstream methods. Dai \etal \cite{dai2014simple} recovered the camera motion and 3D shapes from 2D annotations through rank-3 search and low-rank constraint, and proposed a non-rigid reconstruction method without priori, showing that the low-rank constraint is sufficient to constrain 3D structure recovery. This method was subsequently improved by Kumar \etal \cite{kumar2022organic}, achieving better reconstruction results through organic priors and weight shrinkage operator. Lee \etal \cite{lee2013procrustean, Lee_2014_CVPR} proposed to use procrustean alignment algorithm to eliminate the rigid motion between the 3D shapes, so as to minimize the impact of rotation ambiguity.
% Park \etal \cite{park2017procrustean} followed this idea and proposed a new optimization framework, which was later extended to the field of deep learning\cite{park2020procrustean}. For dense NRSfM task, the mainstream method is to use constraints such as isometry and conformal to model the mapping relationship between two 3D surfaces\cite{parashar2017, parashar2020local}.

\subsection{Deep NRSfM Methods}
Novotny \etal \cite{novotny2019c3dpo} proposed the first deep learning framework for NRSfM. They design a decomposition network to predict shape and motion seperately, and use canonical loss to fix the estimated 3D shapes in the canonical coordinate. Kong \etal \cite{kong2020deep} used the sparse representation assumption to build a hierarchical network for non-rigid 3D reconstruction. Wang \etal \cite{wang2020deep} extended this method to the perspective projection model. Park \etal \cite{park2020procrustean} extended the alignment constraint in Procrustean Regression\cite{park2017procrustean} to the deep learning method, avoiding the complex camera motion estimation problem. Zeng \etal \cite{zeng2021pr} further strengthened the inter-frame structure connection by introducing a regularization constraint for the pairwise alignment of 3D shapes. Wang \etal \cite{wang2021paul} 
% combined deep learning with the traditional optimization method, 
propose to use the orthographic-N-point algorithm to regularize auto-encoder to obtain better reconstruction.  Sidhu~\etal~\cite{sidhu2020neural} designs the trajectory energy function for imposing subspace constraints, accompanied by a regular term for temporal smoothing.  However, the method does not combine subspace constraints with sequential temporal constraints
% These methods all focus on recovering a single, determined 3D structure. 
Recently, Zeng \etal \cite{zeng2022mhr} focused on the depth ambiguity problem and modeled the generation of multi-hypothesis through the introduction of Gaussian noise.

Deep Sparse NRSfM Methods often directly use the network to regress the coordinates of 3D keypoints corresponding to 2D annotations, while 
dense NRSfM tasks often use mesh or implicit nerual representation to represent 3D structures. Yang \etal \cite{yang2021lasr, yang2021viser, Yang_2022_CVPR} proposed a framework that establishes the correspondence between long-sequence observation points by optical flow and model the deformation with skin model. In this paper, we focus on the reconstruction of sparse non-rigid 3D structures.

\subsection{Sequence Modeling}
% Recurrent Neural Network (RNN) was first proposed for sequence-to-sequence regression tasks\cite{rumelhart1986learning, werbos1990backpropagation}. To improve the performance on long sequence tasks, varieties of RNN, such as Long short-term memory(LSTM)\cite{hochreiter1997long} and Gated recurrent unit(GRU)\cite{chung2014empirical}, are capable of learning long-term dependencies. 
The introduction of neural networks in sequence processing problems can improve processing efficiency and has been widely used in many sequence-to-sequence processing tasks\cite{hinton2012deep, krizhevsky2017imagenet, he2017mask}. Recently, the proposal of Transformer \cite{vaswani2017attention} has greatly promoted the development of the sequence modeling network. Transformer and its varieties 
% establish the connection between sequence tokens through the attention mechanism and have achieved great success in processing long sequence tasks. This type of network structure 
has been extended to many other fields, such as human body pose estimation\cite{kocabas2020vibe, zhang2022mixste}, action recognition\cite{choi2019can}, NRSfM\cite{deng2022deep}, \emph{etc}.

Some methods do not adopt the Transformer structure, but try to deal with sequence problems from other perspectives. Wu \etal \cite{wu2022timesnet} used the time series analysis method to calculate the spectrum information of the sequence.
% , and better extracted the periodic information by dividing the long sequence. Aiming at the high space-time complexity of attention, 
Qin \etal \cite{qin2023toeplitz} proposed to use the relative position encoded Toeplitz matrix to replace the attention to realize the function of the tokens mixer. In deep non-rigid 3D reconstruction tasks, some methods strengthen the network's understanding of sequences. Park \etal \cite{park2020procrustean} used the Procrustean alignment to design an optimization equation and extended it to a loss function.
% constrained network to estimate a non-rigid 3D structure sequence. 
Zeng \etal \cite{zeng2021pr} constructed the internal constraints of the 3D structures through pairwise contrastive and consistent regularization.

==> text/3_1GPA_Layer.tex <==
\subsection{General Procrustean Analysis Layer}
\label{sec:GPA}
% In the previous section, we gave the origin of ambiguity in terms of both physical and numerical meanings. The numerical ambiguity is reflected in the underdetermination of the intermediate results when using the classical factorization solution process based on SVD, and this underdetermination reflects the incompleteness of this solution process in terms of constraints, which cannot determine the unique reconstruction results, and the detailed derivation process has been fully elaborated by Xiao \etal~\cite{xiao2004closed}. Meanwhile, the treatment proposed by Xiao \etal is to add new a priori conditions to the basis matrix. However, the additional introduction of a priori will reduce the scenarios in which the method can be applied, and such a more abstract quantitative analysis is also more difficult to lead to new methods.

To reduce the ambiguity described as Eq.~\eqref{eq:motion_ambiguity} for alleviating the loss of accuracy on estimating shapes, we design a computational module $\mathcal{G}: \mathbb{R}^{F\times 3P}\to\mathbb{R}^{F\times 3P}$ that constrains the sequence estimated by the network to the canonical coordinate system originally proposed by C3DPO~\cite{novotny2019c3dpo}.
% \ie~ $\mathbf{\hat{S}}=\mathcal{G}(\mathbf{\tilde S}) ,\mathbf{\hat S} \in \mathcal{S}$. \YC{symbols have not been defined.}
               
\begin{canonical}
    \label{def:canoincal}
    A deforming shape set $\mathcal{S}=\{\mathbf{S}_1,\cdots,\mathbf{S}_n\}$ is in canonical coordinate, $\forall \mathbf{S,S'}\in\mathcal{S}$ and $\mathbf{R}\in\text{SO}(3)$ $\mathbf{S}=\mathbf{R}\mathbf{S'}$ i.f.f. $\mathbf{S} = \mathbf{S'},\mathbf{R}=\mathbf{I}_3$.
\end{canonical}
Unlike C3dpo, we define the input sequence rather than the entire dataset as deforming shape set $\mathcal{S}$.

% A more intuitive way of describing this is shown in Eq.~\ref{eq:motion_ambiguity}. The ambiguity comes from the fact that the motion coupling cannot be uniquely decomposed. Specifically, in the calculation process, we cannot know whether the camera motion $\mathbf{R}_{motion}$ obtained from the decomposition does not contain the motion of the object $\mathbf{R}_{shape}$, and conversely the motion of the object $\mathbf{R}_{shape}$ does not contain the motion of the camera, $\mathbf{R}_{motion}$ and there is no way to distinguish between them due to the lack of conditions. As a fundamental problem at the modeling level, there are solutions to deal with this problem in both traditional and deep learning algorithms. These algorithms may operate in a slightly different way when dealing with ambiguity, but they share a similar idea, namely canonical or alignment.

% Arbitrary pairs of shapes in the set of shapes in the canonical state cannot be transformed to each other by rigid transformation. 
% This definition allows all shapes to be aligned to a common coordinate system, rather than being in their own coordinate system, 
Thus, the previously coupled motion decomposition problem is treated as solving only one motion $\mathbf R_{motion}$. It should be noted that the motion $\mathbf R_{motion}$ here is actually no longer the camera motion but a combination of the origin camera motion and shape rigid motion, $\mathbf R_{motion}= \mathbf R_{camera}\mathbf R_{shape}$, since NRSfM focuses more on the recovery of the nonrigid shapes.
% , this approach of abandoning the recovery of the camera motion is used.

% To reduce the impact of sequence ambiguity, we need to determine the canonical coordinate in which 3D shapes are located. 


\begin{figure*}[t]
  \centering
  % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{5cm}{0cm}}
  \includegraphics[width=0.8\linewidth]{Figs/canonical.pdf}
  \caption{The left side of the figure shows the canonicalization method in \cite{novotny2019c3dpo}, which performs random rotations for each frame, \ie, training the network over the \emph{entire dataset} to determine the canonical coordinate. The right side shows our method to align for \emph{each sequence}, explicitly helping the network to determine the canonical coordinate.}
  \label{fig:canonical}
\end{figure*}


% Seq2Seq~\cite{deng2022deep} built a canonicalization module following \cite{novotny2019c3dpo} from a single-frame perspective to deal with the rotation ambiguity. 
% This Canonical model requires random sampling in the rotation space $\text{SO}(3)$ for each frame of 3D structure in the sequence and training the network to be invariant to arbitrary rotational transformations. In contrast, when using sequence information for canonicalization modeling, each sequence can be aligned by exploiting the similarity between 3D structures of different frames. This approach 
In contrast to another Deep NRSfM classical work C3dpo\cite{novotny2019c3dpo} Seq2Seq~\cite{deng2022deep} differs in that it does not need to random sampling in the rotation space $\text{SO}(3)$ for each frame of 3D shape and training the network to be invariant to arbitrary rotational transformations. The context layer in Seq2Seq granting greater focus on estimating the sequence structure. The specific principle is shown in Fig.~\ref{fig:canonical}.

% To achieve this, we follow the idea used in traditional NRSfM to design the GPA Layer, which models the canonical coordinate by General Procrustean Analysis\cite{gower1975generalized}. 
Inspired by PND~\cite{lee2013procrustean}, PR~\cite{park2017procrustean} and PRN~\cite{park2020procrustean}, we design a parameter-free GPA Layer, which uses Generalized Procrustean Analysis~\cite{gower1975generalized} to model the canonical coordinate and employs an iterative approach to obtain aligned shapes. 
% The GPA layer is a parameter-free module and
The goal of the GPA layer is to eliminate rigid motion between any two frames as much as possible in the least squares sense.
% then the goal of GPA Layer is to find the mean shape $\mathbf{\Bar{S}}$ such that the sequence aligns to it with the least amount of variation. 
The GPA layer takes 3D sequence $\mathbf{\tilde{S}}$ as input and outputs the aligned 3D shapes $\mathbf{\hat{S}}$, which is defined as follows:
\begin{equation}
    \mathbf{\hat{S}} = \mathbf{\hat{R}}\mathbf{\tilde{S}},~ \mathrm{and}~ \left \{ \mathbf{\hat{R}}_{i} \right \}_{i=1}^{F}=\arg \min_{\mathbf{R}_{i}}\sum_{i=1}^{F}\left \| \mathbf{R}_{i}\mathbf{\tilde{S}}_{i} - \mathbf{\bar{S}}\right \|_{F}^{2},
\end{equation}
where $\mathbf{\bar{S}}$ is the mean shape of aligned shapes, which is updated during the iteration, and $\mathbf{\tilde{S}}$ is the reconstructed 3D shape which will be introduced in Sec.~\ref{sec:seq_recon}.
% Then, the aligned shapes can be expressed as $\mathbf{\hat{S}}_{i} = \mathbf{\hat{R}}_{i}\mathbf{S}_{i}$. 
The aligned shapes $\mathbf{\hat{S}}$ are under a fixed coordinate and can naturally be added with some regularization, such as low-rank \emph{etc}.

PRN \cite{park2020procrustean} gives an elegant derivation of how to introduce constraints using GPA in gradient backpropagation, but is accompanied by a high computational overhead. Here we have an approach that is simpler in terms of implementation, but has a similar level of effectiveness. We refer to the iterative gradient backpropagation procedure of \cite{zheng2021ham} and use the one-step gradient strategy to approximate the gradient of the GPA layer during the iteration.

Next we show how the gradient of this computational procedure should be propagated. Suppose that the regularization term constraint acting on $\mathbf{\hat{S}}$ is $\mathcal{G}(\cdot)$, then the gradient can be calculated according to the chain rule similar to \cite{park2020procrustean}:
\begin{equation}
   \frac{\partial \mathcal{G}}{\partial \mathbf{S}} = \left \langle \frac{\partial \mathcal{G}}{\partial \mathbf{\hat{S}}}, \frac{\partial  \mathbf{\hat{S}}}{\partial \mathbf{S}} \right \rangle,
\end{equation}
where $\left \langle \cdot, \cdot   \right \rangle$ represents the inner product. Once $\mathcal{G}$ is defined, $\frac{\partial \mathcal{G}}{\partial \mathbf{\hat{S}}}$ can be directly derived. Since computing $\mathbf{S}\!\rightarrow\!\mathbf{\hat{S}}$ is an iterative process with an unknown number of iterations, we represent $\frac{\partial \mathbf{\hat{S}}}{\partial \mathbf{S}}$ into iterative form according to the chain rule:
\begin{equation}
    \frac{\partial \mathbf{\hat{S}}}{\partial \mathbf{S}} = \left \langle \frac{\partial \mathbf{\hat{S}}}{\partial \mathbf{S}^{k}},\left \langle \frac{\partial \mathbf{{S}}^{k-1}}{\partial \mathbf{S}^{k-2}}, \left \langle \cdots, \left \langle \frac{\partial \mathbf{{S}}^{2}}{\partial \mathbf{S}^{1}}, \frac{\partial \mathbf{{S}}^{1}}{\partial \mathbf{S}}\right \rangle \cdots \right \rangle   \right \rangle \right \rangle
\end{equation}
where $\mathbf{S}^{k}$ is the intermediate state in the iterative process. And this back-propagation process allows the shape sequence $\tilde{\mathbf{S}}$ estimated by our backbone network to be in the canonical coordinate as much as possible.
% To back-propagate the gradient of the iterative algorithm stably, we use the One-Step Gradient strategy proposed in \cite{zheng2021ham}. The regular term can then constrain the sequence estimation module to update the parameters.  
% PRN \cite{park2020procrustean} rigorously derives how to perform gradient backpropagation when using the GPA modules in networks. Here we have an approach that is simpler in terms of implementation, but has a similar level of effectiveness. We refer to the iterative gradient backpropagation procedure of \cite{zheng2021ham} and use the one-step gradient strategy to approximate the gradient of the GPA layer during the iteration.

==> text/3_2Context_Layer.tex <==
\subsection{Sequence Reconstruction}
\label{sec:seq_recon}
% As shown in Eq.~\ref{eq:orgin_BMM}, in the traditional algorithm, it is assumed that any deformation shape can be obtained by a set of basis linear combinations. However, Eq.~\ref{eq:union_subspace} states that the elements in the deformation sequence are not necessarily in the uniform shape subspace. In other words, the deformation sequence is not necessarily represented by a definite number of sets of shape bases, and it is possible that there are several intersecting and merging sets of different shape bases tensor into subspaces at the same time. This means that a linear combination of some shapes in a sequence of deformations should be able to express some other shapes that are in the same subspace:

% \begin{equation}
%     \mathbf{S}_m = a_0\mathbf{S}_0 + \cdots + a_n\mathbf{S}_n, \mathbf{S}_i \in \text{Span}\{\mathbf{B}_1, \cdots ,\mathbf{B}_k\}
% \end{equation}

In the previous section, we introduce the GPA layer, which aims to reduce motion ambiguity by aligning the shape sequences to the canonical coordinate, and in this section, we describe what properties should exist for the sequence. Inspired by Eq.~\eqref{eq:union_subspace}, 
% when there is no constraint (non-zero) \YC{non-zero???} on the coefficient matrix, 
sequence can be represented as follows:
% And for a more general form, without assuming that non-zero weights must be used when performing linear combinations, in other words, no longer confining the shapes to the same subspace, then for the whole sequence of shapes, we can find that there is actually an inherent \textbf{self-expression} property of the whole sequence, by flattening a shape matrix into a vector and representing the sequence in matrix form, then we can obtain
\begin{equation}
    \mathbf{S} = \mathbf{C}\mathbf{S}, \mathbf{S}=[\mathbf{S}^\prime_1,\cdots,\mathbf S^\prime_F]^\intercal, \mathbf{S}^\prime_i\in\mathbb{R}^{1\times 3P}.
\end{equation}

This indicates that any shape can be derived through a linear combination of other shapes. In this form, it is found that the identity matrix $\mathbf{I}$ is a trivial case for coefficient matrix $\mathbf{C}$, \ie~shapes in the sequence are not related to each other. However, the study conducted by \cite{zhu2014complex} indicates that the shapes with close distances in the deformation sequence are present in the same subspace. This guarantees the absence of trivial cases, meaning that the deformation shape sequence obtains the \textbf{self-expressive} property.

To guarantee that the estimated shape sequence has self-expressive properties, we could rebuild the sequence by applying a coefficient matrix connected to it:
\begin{align}
    \mathbf{S} &= \mathbf{C}\mathbf{S}^\prime, \mathbf{C}=\mathcal{H}(\mathbf{S}^\prime), \\~s.t.~~\mathbf{S}^\prime&=[\mathbf{S}^\prime_1,\cdots,{\mathbf S}^\prime_F]^\intercal, \mathbf{ S}^\prime_i\in\mathbb{R}^{1\times 3P}.
\end{align}
% This regularity ensures that the sequences estimated by the network must have the self-expression property. 
% In considering how to construct the mapping $\mathcal{H}(\cdot): \mathbb{R}^{F\times 3P}\to\mathbb{R}^{F\times F}$ of the coefficient matrix, \cite{deng2022deep} constructs the coefficient matrix by measuring the degree of similarity between the shapes, which in turn reconstructs the entire sequence. However, this coefficient calculation takes little account of the temporal information of the sequence.
% However, this way of constructing the coefficient matrix only takes into account the similarity of the shapes but not the distance between the shapes on the sequence. Although, absolute position coding is used in an attempt to add position information to the data in the form of bias, the network may not be able to understand the role played by bias in the absence of downstream constraints.
Where the mapping $\mathcal{H}(\cdot): \mathbb{R}^{F\times 3P}\to\mathbb{R}^{F\times F}$ is referenced from the \cite{qin2023toeplitz}. This mapping is designed to encode shape temporal position and similarity in the coefficient matrix at the same time. To make the network more flexible, we here first map the shapes to the feature space before imposing this regularity:
\begin{equation}
    \label{eq:context_layer}
    \mathbf{\tilde{S}} = g_s(\mathcal{H}(g(\mathbf{S'}), \mathbf{L}, \mathbf\Theta)g(\mathbf{S'})),
\end{equation}
where $\mathbf{S'}$ is the deforming sequence output from the predictor $f_\mathbf{S}(\cdot, \Theta_\mathbf{S})$ in Eq.~\eqref{eq:single_net}, $\mathbf{\Theta}$ is the learnable parameter, $\mathbf{L}$ is a series vector representing the sequence order, \ie~$\mathbf{L}=[1,2,\cdots,F]^{\intercal}$. To make the network more flexible, we impose this constraint in the feature space. $g:\mathbb{R}^{F\times 3P}\to\mathbb{R}^{F\times D}$ maps the shape to the feature space, and $g_s:\mathbb{R}^{F\times D}\to\mathbb{R}^{F\times 3P}$ remaps the deformation sequence from the feature space back to the shape space.

% Eq.~\ref{eq:context_layer} only regularizes the self-expression property that the sequence structure should have, and is not explicit enough to constrain the low-rank characteristics of the deformation sequence, so we use a kernel parametric loss function downstream as a complement to the constraint on the sequence structure:

From the above self-expressive properties of the deformation sequence, it is clear that the shapes in the sequence are linearly correlated with each other. Therefore, the deformation sequence matrix $\mathbf{S}$ should be in canonical coordinate described by Definition~\ref{def:canoincal} and rank defect. Therefore, we perform the canonicalization with GPA Layer and the nuclear norm loss on the shape sequence, $\| \mathbf{\hat{S}}\|_*$. The nuclear norm alone cannot point to the correct learning direction, so we use the re-projection error as a data term, and finally obtain the total loss function that oversees the entire pipeline training process as follows:
\begin{equation}
    \mathcal{L} = \alpha\| \mathbf{W} - \mathbf{\Pi}\mathbf{R}\mathbf{\tilde{S}} \|_2 + \beta\| \mathbf{\hat{S}} \|_*,
\end{equation}
where $\alpha$ and $\beta$ are hyperparameters used to the balance of loss functions. After analysing the results of our experiments, we hereby choose the loss weight as $\alpha=9,\beta=0.1$.





==> text/3_3Implementation.tex <==
\subsection{Implementation Details}

The complete network can be divided into three part. In the first part, we use a single-frame predictor to obtain an intermediate sequence (we here use the predictor structure of C3dpo\cite{novotny2019c3dpo}). In the second part, the intermediate sequence obtained by the single-frame predictor is first mapped to the feature space, and then regularized by the context layer to ensure that the sequence can have the self-expressive property, and then mapped back to the shape space. Finally, the output sequence is then regularized by the GPA layer for ambiguity reduction, and the reprojection error and nuclear norm are calculated using the final output shape sequence for training supervision of the pipeline.

The network module $g$ is a one-layer linear layer, the input dimension is $3\times P$, the output dimension is 128. $g_s$ contains a gated linear unit\cite{shazeer2020glu} and a four-layer MLP. $\mathcal{H}$ contains a gated Toeplitz unit (Gtu) as \cite{qin2023toeplitz}. In addition, the GPA layer is a regularization module used in training and it does not contain any learnable parameters, so that it can be left out of the computation during testing. 
To clearly present the structure of our network module, we have provided more detailed information in our \textbf{supplementary material}. The experimental settings are, GPA convergence threshold is $1e^{-8}$, and the maximum number of iterations is 100. The weight of the loss function is $\alpha=9,\beta=0.1$, the sequence length is 32, the batch is 256, and 4 Nvidia RTX 3080Ti are used for training.

==> text/3_Method.tex <==
\section{Method}


\subsection{Preliminary}
\begin{figure*}[t]
  \centering
  % \fbox{\rule[-.5cm]{0cm}{5cm} \rule[-.5cm]{5cm}{0cm}}
  \includegraphics[width=0.8\linewidth]{Figs/nips_pipeline.pdf}
  \caption{An overview of deep NRSfM pipeline with proposed shape sequence reconstruction and GPA layer. The whole pipeline consists of three part: the single-frame shape/rotation predictor, the shape sequence reconstruction stage and general procrustean analysis layer. The General Procrustean Analysis layer is a parameter-free layer, which is not needed for inference when training is finished. }
  \label{fig:pipeline}
\end{figure*}


We first introduce the definition of this problem and review some classical solutions to provide possible thinking paths. The following equation gives the general form of NRSfM:
\begin{equation}
\begin{aligned}
\label{eq:motion_shape}
\mathbf{W}
% &= \mathbf{\Pi}\left[ \begin{array}{c}
%              \mathbf{R}_1 \mathbf{S}_1\\
%              \vdots \\
%              \mathbf{R}_F \mathbf{S}_F \\
%            \end{array}
%          \right] \\
&= \begin{bmatrix}
\mathbf{\Pi}_{1}  &  & \\ 
 & \ddots  & \\ 
 &  & \mathbf{\Pi}_{F} 
\end{bmatrix} \left[
    \begin{array}{ccc}
      \mathbf{R}_1 &  &  \\
       & \ddots &  \\
       &  & \mathbf{R}_F \\
    \end{array}
  \right]\left[
           \begin{array}{c}
             \mathbf{S}_1 \\
             \vdots \\
             \mathbf{S}_F \\
           \end{array}
         \right]
         \\ &= \mathbf{\Pi}\mathbf{R} \mathbf{S}, \mathbf{W}\in\mathbb{R}^{2F\times P},\mathbf{R}\in\mathbb{R}^{3F\times3F},\mathbf{S}\in\mathbb{R}^{3F\times P},
\end{aligned}
\end{equation}
where $\mathbf{\Pi}_{i}=\begin{bmatrix}
1 & 0 & 0;0 & 1 & 0
\end{bmatrix}$ is the orthogonal projection matrix, $\mathbf{W}$ is the matrix composed of 2D observations of continuously deforming objects, $\mathbf{S}$ is the 3D shape corresponding to the 2D observations, and $\mathbf{R}$ is the motion matrix. 
% The factor decomposition framework is based on the above modeling, and the 3D shape of the target is obtained from the observed data by purposeful decomposition of the 2D observation matrix to achieve the reconstruction. Since nrsfm is more concerned with the reconstruction of the structure than with the recovery of motion, the translation has been eliminated by the centrality of the data in the above modeling. 
It should be noted that in the above modeling, no distinction is made between the ego-motion of the camera and the motion of the object:
\begin{equation}
    \label{eq:motion_ambiguity}
\mathbf{W}=\mathbf{\Pi}\mathbf{R}_{motion}\mathbf{S}=\mathbf{\Pi}\mathbf{R}_{camera}\mathbf{R}_{shape}\mathbf{S}.
\end{equation}

% In a physical sense, it is also difficult to disentangle two motions that are closely coupled without defining a priori the motion of the camera or the object. And from the point of view of numerical characteristics, both motions belong to the special orthogonal group, which is closed to multiplicative calculations, and a motion matrix can be decomposed into the product of any two motion matrices without the introduction of additional conditions, and this arrives at the most important ambiguity problem in nrsfm. 
The underdetermination defect caused by this ambiguity of coupled motion has resulted in the loss of reconstruction accuracy in traditional methods and deep methods, and how to effectively deal with this problem has become one of the focuses of discussion in various works.
% To tackle with this, we propose general procrustean analysis layer for deep nrsfm method to reduce the impact, and a sequence in a uniform coordinate system is more conducive to subsequent analysis.

% In the factorization framework, classical solution framekwork proposed by bregler, it goes a step further and models 3D shapes as a linear combination of a set of shape bases:

% \begin{equation}
%     \mathbf{W}=\mathbf{RS}=\mathbf{R}(\mathbf{C}\otimes\mathbf{I_3}) \mathbf{B}=
%     \left[ \begin{array}{ccc}
%              c_{11}\mathbf{R}_1 & \cdots & c_{1K}\mathbf{R}_F\\
%              \vdots & \vdots & \vdots \\
%              c_{F1}\mathbf{R}_1 & \cdots & c_{FK}\mathbf{R}_F\\
%            \end{array}
%     \right]
%     \left[ \begin{array}{c}
%          \mathbf{B}_1  \\
%          \vdots \\
%          \mathbf{B}_K
%     \end{array}
%     \right]
%     =\mathbf{\Pi B}
% \end{equation}
% where $\mathbf{C}$ denotes a linear combinatorial weight matrix, and $\mathbf{B}$ denotes a set of bases capable of representing arbitrary shapes. 
% % This framework specifies the ideas that can be solved numerically for the above model, but it still cannot solve the ambiguity problem caused by the coupling of camera motion and object motion, and the most direct trouble caused by the ambiguity problem is the underdetermination of the solution process, which eventually leads to the loss of reconstruction accuracy.
% % In this solution process, the model represents the deformation shape in a linear combination though. 
% Specifically, instead of solving each shape basis $\mathbf{B}_i$, this framework solving the motion matrix $\mathbf{R}_i$ first and subsequently solving the shape matrix with the reprojection error as a cost term in an optimization manner (the process can be initialized with a pseudo-inverse). 
% In this model, since the combination matrix $\mathbf{\Pi}\in\mathbb{R}^{3F\times3K}$ and the frame count $F$ is larger than basis number $K$, therefore, $\text{rank}(\mathbf{\Pi})\leq{3K}$. For the basis matrix $\mathbf{B}\in\mathbb{R}^{3K\times3P}$(P is the point number of each shape), the same reasoning leads to $\text{rank}(\mathbf{\Pi})\leq{3K}$. With this as the initial condition, the SVD(singular value decomposition) can be used to obtain the initial \textbf{factors}, $\mathbf{W}=\mathbf{\tilde\Pi}\mathbf{\tilde{B}}, \text{rank}(\mathbf{\tilde\Pi})=3K, \text{rank}(\mathbf{\tilde B})=3K$ , from observation, and then the decomposition result can be adjusted by a gram matrix so that the final result can be obtained as desired:

% \begin{equation}
%     \mathbf{W} = \mathbf{\Pi}\mathbf{B} = \mathbf{\tilde\Pi} \mathbf{G}\mathbf{G}^{-1} \mathbf{\tilde B}
% \end{equation}

% A large body of work builds on the above reasoning and attempts to enhance the accuracy of the final reconstruction result S using various computational techniques. However, \cite{} pointed out that the solution by this method still suffers from numerical underdetermination, and this underdetermination problem can appear in a more hidden form and directly interfere with the reconstruction accuracy, so they added some strong a priori for the selection of the shape basis. But the \cite{} method demonstrates that there is a way to reconstruct the reconstruction results using this inference process while bypassing the associated underdetermination problem. \cite{}, on the other hand, builds on this foundation and successfully constructs a solution algorithm that does not require the addition of additional priors based on the low-rank characteristics embodied in the sequence data itself.

The solution model defined by Eq.~\eqref{eq:motion_shape} is usually transformed into an optimization model with additional constraints, and one of the most representative work\cite{dai2014simple} gives the optimization condition by analyzing the rank of the sequence matrix to suppress ambiguity:
% \begin{equation}
%     \label{eq:orgin_BMM}
%     \mathbf{W} = \mathbf{R}\mathbf{S}, \text{rank}(\mathbf{S}^\sharp)=\text{K}, \mathbf{S}\in\mathbb{R}^{3F\times P},\mathbf{S}^\sharp\in\mathbb{R}^{F\times3P}
% \end{equation}
% where K is the number of bases, and $\mathbf{S}^\sharp$ is the flattened single frame shape sequence matrix. 
% However, since using rank as an optimization condition is an np-hard problem, a relaxation is made in the actual computation, i.e., the rank constraint is replaced by the nuclear norm to make it a solvable optimization problem.
\begin{equation}
    \min_{\mathbf{S}}{\|\mathbf{S}^\sharp\|_*}, s.t. \mathbf{W}=\mathbf{\Pi}\mathbf{RS},\mathbf{S}\in\mathbb{R}^{3F\times P},\mathbf{S}^\sharp\in\mathbb{R}^{F\times3P},
\end{equation}
where $\mathbf S^\sharp$ is a reshuffled form of $\mathbf S$ as described in Dai~\etal~\cite{dai2014simple}. The most important feature of this model is that no additional priori assumptions are introduced for the solution, but rather a low-rank constraint.
% The success of this method practically indicates that the structure of the deformation shape sequence itself has some characteristics that can be exploited to better constrain the solution algorithm.
Later, Zhu~\etal~\cite{zhu2014complex} noted on the basis of Dai~\etal\cite{dai2014simple} that this low-rank constraint on deforming sequences can be extended to a union-of-subspace representation. This work assumes that deforming shapes in the same sequence should come from one or more intersecting shape spaces, each of which is spanned by a set of shape basis:
\begin{equation}
    \min_{\mathbf{D}}{\|\mathbf{D}\|_*}, s.t. \mathbf{W} = \mathbf{\Pi}\mathbf{R}\mathbf{S}, \mathbf{S} = \mathbf{D}\mathbf{C},
        \label{eq:union_subspace}
\end{equation}
where $\mathbf{D}$ is a dictionary matrix containing multiple bases that can be tensed into different subspace shapes, and $\mathbf{C}$ is a coefficient matrix. This sequence modeling method referred to LRR\cite{liu2012robust} brings new effective constraints to the solution process, refining the regularity of the low-rank constraint on the estimation results.

% We find that the above two regular patterns each construct the constraints required for sequence modeling of the nrsfm problem from different perspectives, extracting properties of the sequence structure from different aspects and using them to assist the reconstruction process, 

However, these modeling of sequences are rarely discussed in subsequent deep methods, and the mainstream deep methods~\cite{novotny2019c3dpo,kong2020deep,wang2021paul} reconstruct the non-rigid shape sequences in a \emph{single-frame lifting} way as follows:
\begin{align}
    \label{eq:single_net}
    &\mathbf{S'}_i = f_{S}(f(\mathbf{W}_i),\Theta_{\mathbf S}), \mathbf{S'}_i \in \mathbb{R}^{3\times P},\\
    &\mathbf{R}_i = f_{R}(f(\mathbf{W}_i),\Theta_{\mathbf R}), \mathbf{R}_i \in \mathbb{R}^{3\times3},
\end{align}
where $\Theta$ is learnable parameters, and $f:\mathbb{R}^{3\times P}\to\mathbb{R}^{D}$ is an encoder module. Whilst such methods heavily rely on a network's ability to recall the relevant 3D structure from a sole frame of data, it is evidently apparent that they are incapable of utilizing constraints from \emph{sequence context, temporal information, and the sequence structure itself} which can be provided to facilitate the reconstruction process.

In this paper, we revisit the canonicalization and the sequence structure self-expressive regularity under sequence modeling, and design modules that can effectively impose both constraints to obtain a deeply non-rigid reconstruction pipeline that can effectively exploit the sequence structure information. The entire pipeline is shown in Fig.~\ref{fig:pipeline}, and we will then present first how to perform canonicalization in Sec.~\ref{sec:GPA}, followed by sequence modeling in Sec.~\ref{sec:seq_recon}.
% we propose two modules capable of reducing the ambiguity and  the total pipeline is shown in Fig.~\ref{fig:pipeline}, turning the previous single-frame estimation into a sequence-to-sequence deep non-rigid reconstruction pipeline that can efficiently exploit the sequence structure properties.



==> text/4_4Discussion.tex <==
\section{Discussion}\label{sec:discussion}

\begin{table}[t]

%  It can be seen that GPAlayer is not as effective on datasets with shorter sequences as it is on longer datasets.}

\small
  \tabcolsep=0.28cm
\centering
\begin{tabular}{c|ccc}
\toprule
            & Seq2Seq & \textit{Seq2Seq with GPA} & Ours  \\ \hline
CMU-S23-All & 0.137       & 0.209                & 0.168 \\ 
CMU-S34-All & 0.142       & 0.232                & 0.201 \\ 
H36M        & 79.8        & 75.6                & 66.1  \\ 
\bottomrule
\end{tabular}
\caption{We show the results of the ablation experiments, where \textit{Seq2Seq with GPA} represents the results of removing the canonical loss in the GPA Layer based on Seq2Seq. This shows the limitation of GPA Layer on datasets with shorter sequence length.}
% \vspace{-0.5cm}
\label{tab:conform}
\end{table}

The difference in results between Table 1 and Table 2 of main text highlights the advantages of our GPA layer on longer sequence data and the limitations on slightly shorter sequence data.  In this section, we discuss about the limits and scope of different alignment regularization terms. We begin this discussion by attempting to answer why Table 1 and Table 2 of main text do not conform over comparing methods. 

The canonicalization loss used by \cite{novotny2019c3dpo} is an implicit regularization term that obtains alignment results over the entire dataset. This approach is more effective for shorter sequences or smaller datasets. However, for larger datasets, this \textbf{global alignment} becomes a bottleneck. We believe that a better approach in this case is to perform the alignment operation for each sequence individually.

However, there are some limitations to this \textbf{local alignment}. If the dataset is overall small, or if the length of each sequence in the dataset (not the input sequence) is short, then the two approaches will not show significant differences. Furthermore, if the dataset has more fragmented data, resembling a ``set'' rather than a ``sequence'', then the dictionary-based approach can also achieve better performance. To verify the idea, we conduct a analysis on the experiment results and perform ablation experiments.

\paragraph{Established Experiments.} As demonstrated in Table 1 in main text, for larger datasets like Human3.6M, Interhand2.6M, the method proposed in this paper that employs GPA Layer for local alignment substantially improves on the canonical loss method (C3dpo and Seq2Seq). Conversely, for smaller datasets like CMU Mocap shown in Table 2 in main text, the overall performance of the local alignment method seems to be similar to that of the global alignment method. If the unseen data is not incorporated into the training process, then employing the global alignment approach with canonical loss yields marginally superior outcomes.

\paragraph{Additional Experiments.} We conduct an ablation experiment to investigate the influences emanating from diverse alignment schemes. We chose two fundamental sequences from the CMU Mocap dataset and the H36M dataset as the test data. The three sets of experiments we devised are as follows: first, we tested the original Seq2Seq; second, we applied GPA Layer to replace the canonical loss of it; and finally, we introduced our proposed method for comparison. The result is shown in Table~\ref{tab:conform}. In this table, \textit{Seq2Seq with GPA} denotes that we replace the canonicalization loss in \cite{deng2022deep} with the GPA layer, and we can see that in doing so, \cite{deng2022deep} achieves comparable results on H36M, while it fails to achieve better result than the original Seq2Seq on the CMU dataset. For analogous reasons, outcomes arise for denser datasets with less data as shown in Table~\ref{tab:short_sequence}.

From the results, their advantage on small datasets is also not that significant, and our results are comparable to theirs. On the other hand, it can be seen that GPA layer is not as effective on datasets with shorter sequences. This aspect serves as a constraint of the methodology suggested in this paper. Specifically, when dealing with a lesser quantity of data, the methodology puts forward in this research does not yield superior outcomes, thereby necessitating further investigation in our future work.


